Youth WellTech: A Global Remote Co-Design Sprint for Youth Mental Health Technology

Mental health is a pressing concern in today's digital age, particularly among youth who are deeply intertwined with technology. Despite the influx of technology solutions addressing mental health issues, youth often remain sidelined during the design process. While co-design methods have been employed to improve participation by youth, many such initiatives are limited to design activities and lack training for youth to research and develop solutions for themselves. In this case study, we detail our 8-week remote, collaborative research initiative called Youth WellTech, designed to facilitate remote co-design sprints aimed at equipping youth with the tools and knowledge to envision and design tech futures for their own communities. We pilot this initiative with 12 student technology evangelists across 8 countries globally to foster the sharing of mental health challenges and diverse perspectives. We highlight insights from our experiences running this global program remotely, its structure, and recommendations for co-research.

==> sections/old_section/01_intro_backup_oct03.tex <==
\iffalse
start off with problems

According to the World Health Organization (WHO), approximately 20\% of the world's children have a mental health condition~\cite{WHO?}, and suicide is the second leading cause of death amongst 15-29 year-olds~\cite{WHO?}.
Many scholars have attributed the prevalence of youth mental health issues to the growing significance of technology~\cite{} in their lives that may amplify social comparison~\cite{} and technology addiction~\cite{} through designs that capture youth's attention and promote endless engagement~\cite{}.
% With the growing significance of technology in the youth's everyday lives, it raises concerns about their well-being.  With suicide rates through the roof due to social comparison, addiction, social media apps are designed to keep you on their site, students scrolling for the next digital high, the list goes on. 
On the other hand, others argue that technology can also provide many benefits to youth~\cite{} such as providing them with the ability to work remotely with others around the world~\cite{}, offering educational and career opportunities~\cite{}, and giving them a platform to raise their voice~\cite{}. 
% Technology causes harms, however inversely there are many benefits to tech, the spread of knowledge, the ability to work remotely with others around the world, offering educational and career opportunities. 
Today's youth has been navigating the good and the bad of growing up emersed in technology. 
Therefore, it is imperative that we involve youth in the design, research, and development of technology.
% It is important that we involve youth in our research, not only as subjects, but researchers too.

Co-designing with youth and actively involving them in the design process is not new~\cite{examples of MH codesign}. 
% People have done co-design, which is a design approach that actively involves end-users in the design process. 
Co-design encourages the flow of ideas between diverse groups of people, stimulating ideas and promoting discussion which may otherwise be overlooked due to bias of an independent researcher~\cite{co-design seminal paper?}. Co-design blurs the lines between researchers and participants, where the participants become researchers, introducing an additional layer of potential participants. 
Co-design has been shown to be a successful approach to tackling the complex intricacies, edge cases, and nuances in society that are challenging to cover through traditional methods and testing~\cite{O'Brien2020A}. 
Even if no benefits arise from the [placeholder], it improves the community itself, specifically in cases of improving mental health \cite{O'Brien2020A}.
% It is clear that co-design is a successful approach to tackling the complex intricacies, edge cases and nuances in society that are not possible to cover through traditional methods and testing, and even if no benefits arise, it improves the community itself, specifically in cases of improving mental health \cite{O'Brien2020A}. 
Co-designing with youth has shown additional benefits in developing novel design features and gaining insights into adolescent attitudes towards various scientific concepts, such as [placeholders]~\cite{Bonsignore2016Traversing}. 
% Co-design has been done with the youth and benefits have been shown, for example \cite{Bonsignore2016Traversing} showed that developing with teenagers resulted in novel design features and gave insight into adolescent attitudes towards various scientific concepts. 
Additionally in the context of the software industry, co-design has been beneficial, in this example adolescents with ASD were able to help in an iterative co-design process \cite{Zhu2019Co-designing}. 

% What's lacking in other work: (1) cross-cultural aspect --> remote, (2) tech as the focus, (3) focus on youth as designers
What seems to be lacking from all of these studies however, is the use of co-design with the youth, cross-culturally, to address mental-health by using technology as the solution, whilst additionally putting more focus on them as the designers. Additionally there is a lack of studies which demonstrate co-design done remotely. It is important to work in an integrated manner with people cross-cultrually when addressing mental health \cite{James2002Cultural}, which can be addressed with co-design, partly due to the massive differences that mental health can bring in different countries as shown amongst university students by \cite{Ochnik2021A}. It is increasingly important that solutions are built for the youth, with the youth in-mind, as shown by \cite{Fusar-Poli2019Integrated} who raised that the youth 12-25 need friendly mental health services that are sensitive to their clinical, neurobiological and psychological development. We really need to get experts amongst the youth, who are at the forefront of technology to build solutions to tackle mental health, as they are the demographic that are going through this rapid increase, especially since many of the youth have gone through the Covid-19 pandemic which has caused multifarious adverse effects on the mental health of the youth \cite{Hawes2021Increases}. There is a huge learning opportunity to learn from the future leaders of society who are innovating with tech every day.

% What we're doing differently: (1) diverse, (2) educate, (3) co-research,
To address this we need to co-design with the youth from around the world so we get a diverse set of perspectives. Not only do we need to just work with the youth to get their opinions, we need to educate, co-research and guide them so they can be involved in the entire interactive design process from start to finish. 
% Goal of running this again in the future
We need students who are passionate about mental health and well being and are driven to solve problems in this space, whilst at the same time we need to be able to get reflections from our youth participants so we are able to run similar co-design research programs like this in the future.

In this case study, we describe our experience of conducting a remote, 8-week collaborative/participatory research program with students at the forefront of building technologies from 8 countries in a program called Youth WellTech. What is novel about our program is that we not only co-designed with our students, but we co-researched with our students and we were able to conduct our program entirely virtually, with students joining remotely from 8 different countries around the world. We went through a human-centered design process from problem identification to designing and prototyping, where the youth presented their ideas to Microsoft employees. Our co-design research contributes to the wider research in many ways: co-designing with the youth to solve mental health and well-being problems with a diverse set of students remotely, learnings and suggestions for how to improve co-design research in the future, and how to run such studies going forward.
\jina{Add the biggest takeaways}
\fi

% (1) youth MH issue is real and serious
The mental health of today's youth is a pressing concern, underscored by alarming statistics. According to the World Health Organization (WHO), one in seven 10-19 year-olds globally experience mental health concerns, many of which go unrecognized and untreated ~\cite{WHO?}. Furthermore, the COVID-19 pandemic has exacerbated these concerns. A 2021 meta-analysis of 29 studies ~\cite{Jama network} found symptoms of depression and anxiety to be "significantly higher" following the onset of the pandemic.
% https://www.who.int/news-room/fact-sheets/detail/adolescent-mental-health#:~:text=Globally%2C%20one%20in%20seven%2010,disease%20in%20this%20age%20group.
% https://info.mstservices.com/blog/global-youth-mental-health

% (2) youth are rarely involved in design of solutions
Despite the gravity of the situation, the youth – those directly affected – are often sidelined in the design and implementation of solutions. Their firsthand experiences make them invaluable contributors to the design, research, and development of technology. It's not just about involving the youth; it's about the principle of "youth designing for youth, precisely because they understand the nuances of being youth."

% (3) co-design is a thing that people have been doing, and it has evolved over the years
Co-design, a collaborative approach to problem-solving, has emerged as a promising avenue to bridge the gap in addressing youth mental health issues. By actively involving all stakeholders, co-design aims to create more relevant and effective solutions. The concept of co-designing with youth is not novel. Over the years, it has been shown to be a successful approach to tackling the complex intricacies in society that are challenging to cover through traditional methods and testing ~\cite{co-design_history}.

% (4) but there are challenges/gaps like not being global or requiring in-person interactions, etc
While co-design has its merits, there are areas that have been less explored. One notable area is the cross-cultural aspect. Most co-design programs are localized, focusing on a particular region or culture ~\cite{local_co-design}. However, a truly global co-design program that is both remote and cross-cultural is rare. Another distinctive gap is the lack of focus on technological innovation. Unlike many co-design initiatives, our participants are not just technically adept but are at the forefront of technology ~\cite{tech_gap}. Their deep technical understanding allows them to conceive innovative solutions using technology. Furthermore, while traditional co-design often sees researchers taking the lead, our approach champions "Youth Driven Technology Design", empowering the youth with more ownership. It embodies a design philosophy driven by the youth, for the youth, and through the youth, ensuring that their voices are not just heard but are central to the design process.

% (5) present our approach to reduce this gap
Building on the identified gaps, our study takes a unique direction. Central to our initiative is the direct involvement of the youth, not merely as participants but as co-researchers. In this endeavor, we collaborated with Microsoft Learn Student Ambassadors, a diverse cohort of students who are not only passionate about technology but also deeply invested in social impact and education.

% (6) our contributions
However, with these unique approaches come challenges. The transition to remote communication, especially in the context of the global pandemic, amplifies certain issues. One pronounced challenge is the difficulty in reading and responding to social cues in an online environment ~\cite{online_communication}. For youths, existing social barriers, such as the fear of judgment or reluctance to voice disagreements, can be magnified ~\cite{youth_barriers}. Additionally, the presence of a diverse cohort introduces layers of complexity. For instance, the interplay between Asian and Western communication styles might introduce cultural barriers ~\cite{communication_styles}.

Moreover, the limitations of previous co-research endeavors provide valuable lessons. Tokenism, where participants are merely symbolic without genuine involvement, can dilute the essence of co-research ~\cite{tokenism}. Power dynamics can persist, making participants, especially youths, hesitant to voice their opinions ~\cite{power_dynamics}. Insufficient training can leave participants feeling ill-equipped, while cultural insensitivity can lead to misunderstandings or even offense ~\cite{training_issues}.

With these considerations in mind, the pressing question arises: How can we effectively conduct co-design with a remote and diverse cohort of youths, ensuring meaningful participation, addressing cultural nuances, and navigating these challenges?
In this paper, we present a comprehensive case study of our co-design program, detailing our processes, encountered challenges, and the invaluable lessons learned. Our co-design research not only contributes a unique perspective by actively involving the youth in addressing mental health and well-being challenges but also offers a diverse, remote collaboration with students from varied backgrounds. Furthermore, our findings provide actionable insights and recommendations for refining co-design research methodologies in the future, setting a precedent for how such studies can be effectively conducted moving forward.
\iffalse
^1^ Placeholder for a citation on the significance of youth mental health.
^2^ Placeholder for a citation on the lack of youth involvement in solution design.
^3^ Placeholder for a citation on the principles of co-design.
^4^ Placeholder for a citation on the benefits of remote communication and diverse problem-solving.
^5^ Placeholder for a citation on the advantages of diversity in co-design.
^6^ Placeholder for a citation on the difficulty of online social cues.
^7^ Placeholder for a citation on cultural barriers in communication.
^8^ Placeholder for a citation on tokenism.
^9^ Placeholder for a citation on power dynamics.
^10^ Placeholder for a citation on training in co-research.
^11^ Placeholder for a citation on cultural insensitivity.
^12^ Placeholder for a citation on challenges in co-design.
^13^ Placeholder for a citation on the unique approach of involving youth as co-researchers.
\fi

==> sections/old_section/01_intro_outline.tex <==
\section{Introduction} %Salman

Probably about 1 page. 

%% group think?


%% background and then the intro, details in background

New outline for intro:

- establish mental health in the first place

% First paragraph: Why co-design
% Fist sentence I'm not so sure about, I've seen a variety of styles:
% \begin{itemize}
%     \item Can start with a hook, a question such as: With the digital-drug, social media, online pressure, distractions at the fingertips of our youth at the inception of their existence on Earth, [how are we going to improve mental-wellbeing if we don't involve them in the design process?] 
    
%     \item Mentioning how social media is designed to keep people longer on the platform, therefore it is increasinly problematic)
%     \item Talking about what co-design is.
%     \item Another paper in the second sentence seems to dive into what the paper is about. We could for example say: Mental health is on the rise with youth, In this co-design study we worked with our students to come up with a solution that keeps them at the centre of design.
% \end{itemize}


half intro summsirze related works and then talk about what we did

First paragraph paint the problem
- MH is an issue
- It's especially an issue for youth in various ways
- Many solutions have been introduced and used
- Youth is rarely involved 
- Involving youth is an important thing

why mental health and well being (touch upon in the first sentence that we're using co-design to connect to the first paragraph.
\begin{itemize}
    % \item In this case-study we use co-design to tackle youth mental health and to increasing well being.
    \item Mental health is increasing amongst the youth: e.g. background research part I mentioned this: According to the World Health Organization (WHO), approximately 20\% of the world's children have a mental health condition, and suicide is the second leading cause of death amongst 15-29 year-olds.
    however technology helps to hav a voice
   
\end{itemize}

Second paragraph
- People have done co-design: describe codesign
If going with why co-design:
\begin{itemize}
    \item Co-design (CD) encourages the flow of ideas between diverse groups of people, stimulating ideas and promoting discussion which may otherwise be overlooked due to bias of an independent researcher.
    \item Co-design blurs the lines between researchers and participants, where the participants become researchers, introducing an additional layer of potential participants.
    \item Clear that co-design is a successful approach to tackling the complex intricacies, edge cases and nuances in society that are not possible to cover through traditional methods and testing.
\end{itemize}
- talk about others who have tried this in ways ABC 
(lack of contribution as a challenge for us that we solve in this study)
- But they lack in ABCD
-  \item Research gap of lack of co-design studies with a global perspective of students who are at the forefront of technologies
youth fighitng tensino, take advantage to use tehcnology to support metnal heatlth


- We really to...position // what needs to be done to remove this gap

TO DO: NEED TO JUSTIFY NOVELTY BEFORE STATING NOVELTY, CHANENL TO BRAODCAST IDEAS IS A GOOD IDEA, normally done with ocmmutiy activists

Third (novelty) - positioning our contribution in HCI

- our aim (to address the challenge we just mentioned)
- To achieve this aim, we need to ABCD. (digital/remote, diverse therefore we need a global group, co-design but co-research and education, teaching so that they can take part in the HCI process rather than being part of the process, and also asking them to reflect to improve the process is lacking in existing), high level as many asepcets as possble


Fourth paragraph: describing what we did - talk about contributions to HCI
\begin{itemize}
        \item in this case study, we describe our experience of conducting an remote, 8-week collaborative/participatory research program with students at the forefront of building technologies from 8 countries in a program called Youth WellTech (here, bring information that highlights our novelty mentioned above.)
    \item describe briefly what that looked like: went through HCD process from problem identification to design to prototyping.
    \item Brief one sentence saying how we contribute: we contribute our lessons learned from conducting such program in runnign the program, structuring the program, and co-research.
    % \item Different key areas we contributed in.
\end{itemize}

    \item Touch on some high level details: We at Microsoft and a group of Gold Microsoft Learn Student Ambassadors from X number of countries (not sure how to introduce this, in laymans terms or with the title? in the introduction) in a fully virtual format over 8 weeks.
    \item Given that we are studying youth mental health and well-being, it was vital to us to work with many students around the world with diverse perspectives, especially ones that just had to deal with the Covid-19 pandemic, to understand how they coped under immense pressure and a change of circumstances, etc.
\end{itemize}







\item Stats of how dangerous the fast the growth of metal health amongst the youth is, or it can stay in the second paragraph.
\item scholars have started, etc. designing with youth
\item mention novelty







\textbf{Context/Background}
% \textbf{Context/Background}: Write a few sentences about the broader context of the work. This could be about the general field of technology for mental health, the specific issues that the co-design activity was trying to address, or the importance of the topic. 


Students around the world are suffering from mental health problems and a lack of proper wellbeing, especially since the pandemic \cite{Garner_2021}. In the digital age, not only do students have to battle and fend of the destructive measures in the environment around them, but also the harm that permeates through the digital world as well \cite{Anna_Lembke1, AnnaLembke0}, such as dopamine, Whilst there are numerous solutions available, we aim to learn from a variety of Gold Microsoft Learn Student Ambassadors, who are uniquely positioned in such a way that they not only manage their university studies, but also present and run workshops or events on top of their everyday lives. They are at the forefront of technology and work cross-disciplinary with and target many different students from around the world. Our cohort spans across many different regions and we ran a co-design study to get inputs from them, the subject matter experts for their universities, and regions. Findings from the study helps us understand what works, what are problems that still need to be solved, and we also are able to understand how to more effectively run more co-design studies going forward. 

There have been many approaches to improving the livelihood of the public, through research done by many independent researchers. Co-design allows us to look collaboratively as a group of researchers to hypothesize, investigate, design and find results as a collective which we may not have been able to do as independent researchers.  

%% 

\textbf{Problem Statement}: Identify the specific problem that this study/paper aimed to address. This could involve an explanation of why current solutions or approaches are inadequate and the need for a new approach. Try to avoid tackling youth mental health crisis as the problem. While that's an important problem, it's too big of a scope. 

\textbf{Purpose of the Study}: Clearly state the purpose of the study/paper. This might be to investigate the experience of participating in a co-design activity, to evaluate the outcomes of the co-design process, or to develop recommendations for future co-design activities.

In this work/study we aim to figure that out by bringing in students from across diverse cultures who interact with and advocate for technology on a daily basis so that they can voice their opinions and contribute to a better wellbeing. Quite often you will find co-design studies that are done local to the specific region, due to constraints of universities, fundings and convenience, by facilitating the co-deign sprint online, we were able to let students contribute to the study from the comfort of their own home, which may enable unique ideas to naturally flow. 

In this work/study, we aim to ... 

\textbf{Unique Contribution}: Identify what new insights or perspectives the case study will provide.  

The main objective of this co-design activity was to get the viewpoints of the youth to co-design for the youth. In other words, our youth group where Microsoft Learn Student Ambassadors that are widely distributed across the world. Through this approach we were able to empower the youth with human-centered design skills, to let their voices be heard voiced and to develop a future pipeline and process for an ongoing partnership with the youth to address youth mental health and well-being technology. Understanding their unique perspective that they have acquired, being both advocates for technology and students growing up through various tough situations, be it Covid-19, the rise in Artificial Intelligence and being around the digital drug known as social media as Anna Lembke calls it. The Microsoft Learn Student Ambassador Gold cohort are uniquely positioned, in that they are actively designing, creating, making, they are are the future CEOs, engineers and leaders of society. 

%Ways to differentiate: 
Whilst there are co-design studies done remote \cite{Sanoubari_2021}, and studies on how we can improve the mental health of the youth using digital technology \cite{Garner_2021}, there does not seem to be a mix of the two. There do seem to be studies done with co-design however using vitual reality, however that is far-fetched and in reality, no-where near mass adoption. What happened recently was an uprorar in how reliant everyone has become on technology, however there has been a lack of studies cross-cultuarly to focus on how to use this technology responsibly. 

%How does this work contribute to existing literature?  
- no bias in the kind of mental health problems we were trying to tackle, avoiding any preconceived schemas or biases


%Why hasn't this been done before?  

%What's wrong with previous approaches? 

%How does our approach differ?  

This could involve new findings about the process of co-design, the role of youth in co-design, or the impact of co-design on technology for mental health. 

\textbf{Study Overview}: Give a brief overview of the study - the methods used, participants involved, and key findings. They should also hint at the implications of the findings, which will be detailed in the conclusion of the paper. 

==> sections/old_section/02_background.tex <==
\section{Background and Motivation} % motivation % Salman/Chino

\todo{We will merge this into the introduction}
% Make it concise
% Make it less about Microsoft advertisement
% Read the introduction and highlight key points like (1) cross-cultural, (2) involving tech innovators, (3) ownership 

% Why youth and mental health
Mental health is increasingly a concern amongst the youth. Quite frankly, it is alarming that over time, the prevalence and impact of youth mental health are not that widely focused on. The youth today are our future leaders, and \textbf{what are they filled with?} social media apps where the digital drug, known as social media, is becoming the source of the next opioid epidemic. According to the World Health Organization (WHO), approximately 20\% of the world's children have a mental health condition, and suicide is the second leading cause of death amongst 15-29 year olds. 
Despite these statistics, the global response to the issue is inadequate. There is a lack of initiative from governments, institutions, schools, colleges, and companies as the global median health expenditure that goes towards mental health is less than 2\%~\cite{to be confirmed after going through source}. So, it is clear that a solution is not coming from the top down any time soon.~\cite{Sounds bit concluding} Evidence shows that mental health is worsening over time, and technology is not helping, or is it? Whatever the case is, it is unlikely that a top-down solution will emerge in the near future. What better way to tackle this, than with the help of the youth themselves? Several studies have demonstrated that technology itself is detrimental to mental health \cite{Chowdhury_2023}. However, eliminating the use of technology is not a feasible solution. Moreover, technology is becoming ever more imperative to use. The gap in technology access and skills contributes to the gap in knowledge and opportunities, which is accelerated due to the rise of advanced technologies such as ChatGPT, Llama 2, and Bard.

We co-designed with Microsoft Learn Student Ambassadors, who are 18 years old and older, to improve the well-being of our youth. They are a global and diverse cohort of students from around the world with diverse backgrounds, cultures, and interests, united by a common goal and passion for technology, social impact, and enthusiasm to teach others. Specifically, we recruited Gold Microsoft Learn Student Ambassadors who are well-versed in the latest and most innovative technologies, as well as have experience in community engagement and advocacy, with the increased usage of technology due to the COVID-19 pandemic. Our goal is to establish a long-term partnership, pipeline, and potentially longitudinal study to help address youth mental health issues to enhance the well-being technology and lives of the youth today and the future youth. A key advantage of working with student ambassadors is that they serve as a link between Microsoft and their local communities. Rather than running a cross-cultural study from a central organization, Microsoft, we were able to have students run their prototypes and designs through their own cohort in a culturally appropriate and non-intrusive manner, reducing the chances for bias in the way students behave, demand characteristics from them and their participants that they recruit. Furthermore, the student ambassadors themselves, who were new to HCI/HCD and UX design, had less researcher bias, since they came in with fresh perspectives of their own, and had no preconceived expectations or desired outcomes that they were aiming to achieve through the study. There are significantly fewer studies done in a co-design manner, and typically these are done in person, as students at university are physically bound by their campus. This inherently puts a bias towards the results that are gathered from most co-design studies and ignores the influence of the digital literacy that the youth of today's society has adopted, as well as educational institutions and the future of the workplace. Not only is this just a remote study, but this is done internationally too, allowing diverse perspectives to surface that otherwise would have been missed in other co-design studies.

Inclusion is a vital aspect of our society, and it plays a crucial role in building products that cater to a diverse set of people, as well as involving a diverse set of people in the process. As Jenny Lay-Flurrie says: nothing for us, without us. Global collaboration enhances the relevance, acceptability, and usability of the technology. A common challenge in research is the applicability and generalisability of the outcomes/findings. If we run a study on just students in Seattle for example, then we cannot with confidence have any replicability in India. By having both researchers and end-users distributed globally, we were able to gain a more generalizable outcome. Additionally, having a global cohort enabled us to tap into the unique, and diverse experiences of young people, allowing their voices, choices, and expectations to be met, regardless of their social status, background, and race. At Microsoft we aim to help every person and organization on the planet to achieve more, and how can we do that without engaging with students distributed globally.

The focus on youth as a target population for research has come up in several areas. In our mental health workshop, experts in the field highlighted the youth mental health crisis where traditional digital or non-digital mental health solutions are inadequate for meeting their needs. The same focus can be seen in the US Surgeon General’s report on youth mental health [1]: they encourage technology companies to challenge the traditional notion of engagement and they ask employers to provide age-appropriate well-being support. In multiple GenZ research conducted by GWS [2] and Research and Insights teams, mental health support is the number one priority that the youth employees seek in the workplace. As digital natives, current and future youth have unique mental health needs that are not being adequately addressed by current solutions [3]. As a company that values human empowerment and as we think about what it means to “create renewable human energy (– Kathleen Hogan)”, the youth population is a crucial investment opportunity for the future. 


==> sections/old_section/02_backgroundold.tex <==
\section{Background and Motivation} % motivation % Salman/Chino


% Why youth and mental health
Mental health is increasingly a concern amongst the youth. Quite frankly, it is alarming that over time, the prevalence and impact of youth mental health are not that widely focused on. The youth today are our future leaders, and what are they filled with? social media apps where the digital drug, known as social media, is becoming the source of the next opioid epidemic. According to the World Health Organization (WHO), approximately 20\% of the world's children have a mental health condition, and suicide is the second leading cause of death amongst 15-29 year olds. 
Despite these statistics, the global response to the issue is inadequate. There is a lack of initiative from governments, institutions, schools, colleges, and companies as the global median health expenditure that goes towards mental health is less than 2\%. So, it is clear that a solution is not coming from the top down any time soon. Evidence shows that mental health is worsening over time, and technology is not helping, or is it? Whatever the case is, it is unlikely that a top-down solution will emerge in the near future. We co-designed with Microsoft Learn Student Ambassadors, who are 18 years old and older, to improve the well-being of our youth.

% reference: https://www.who.int/health-topics/mental-health#tab=tab_2

% Why codesign with students
What better way to tackle this, than with the help of the youth themselves. Several studies have demonstrated that technology itself is detrimental to mental health \cite{Chowdhury_2023}. However, eliminating the use of technology is not a feasible solution. Moreover, technology is becoming ever more imperative to use. The gap in technology access and skills contributes to the gap in knowledge and opportunities, which is accelerated due to the rise of advanced technologies such as ChatGPT, Llama 2, and Bard.

% Why ambassadors
In this study, we collaborated with Microsoft Learn Student Ambassadors. They are a global and diverse cohort of students from around the world with diverse backgrounds, cultures, and interests, united by a common goal and passion for technology, social impact, and enthusiasm to teach others. Specifically, we recruited Gold Microsoft Learn Student Ambassadors who are well-versed in the latest and most innovative technologies, as well as have experience in community engagement and advocacy, with the increased usage of technology due to the COVID-19 pandemic. Our goal is to establish a long-term partnership, pipeline, and potentially longitudinal study to help address youth mental health issues to enhance the well-being technology and lives of the youth today and the future youth. A key advantage of working with student ambassadors is that they serve as a link between Microsoft and their local communities. Rather than running a cross-cultural study from a central organization, Microsoft, we were able to have students run their prototypes and designs through their own cohort in a culturally appropriate and non-intrusive manner, reducing the chances for bias in the way students behave, demand characteristics from them and their participants that they recruit. Furthermore, the student ambassadors themselves, who were new to HCI/HCD and UX design, had less researcher bias, since they came in with fresh perspectives of their own, and had no preconceived expectations or desired outcomes that they were aiming to achieve through the study. 

% Why global participation
Inclusion is a vital aspect of our society. It is essential for products to be built with a diverse set of people, and for a diverse set of people. As Jenny Lay-Flurrie says: nothing for us, without us. Global collaboration enhances the relevance, acceptability, and usability of the technology. A common challenge in research is the applicability and generalisability of the outcomes/findings. If we run a study on just students in Seattle for example, then we cannot with confidence have any replicability in India. By having both researchers and end-users distributed globally, we were able to gain a more generalizable outcome. Additionally, having a global cohort enabled us to tap into the unique, and diverse experiences of young people, allowing their voices, choices, and expectations to be met, regardless of their social status, background, and race. At Microsoft we aim to help every person and organization on the planet to achieve more, and how can we do that without engaging with students distributed globally? 

% Why remote? Not many co-design studies are done remotely and often are done in person
There are significantly fewer studies done in a co-design manner, and typically these are done in-person, as students at university are physically bound by their campus. This inherently puts a bias towards the results that are gathered from most co-design studies and ignores the influence of the digital literacy that the youth of today's society has adopted, as well as educational institutions and the future of the workplace. Not only is this just a remote study, but this is done internationally too, allowing diverse perspectives to surface that otherwise would have been missed in other co-design studies.


\jina{Why youth <--- in case this is helpful, I (Jina) copied this from our original proposal}

Youth mental health is a priority for Microsoft. The focus on youth as a target population for research has come up in several areas. In our mental health workshop, experts in the field highlighted the youth mental health crisis where traditional digital or non-digital mental health solutions are inadequate for meeting their needs. The same focus can be seen from the US Surgeon General’s report on youth mental health [1]: they encourage technology companies to challenge the traditional notion of engagement and they ask employers to provide age-appropriate well-being support. In multiple GenZ research conducted by GWS [2] and Research and Insights teams, mental health support is the number one priority that the youth employees seek in the workplace. As digital natives, current and future youth have unique mental health needs that are not being adequately addressed by current solutions [3]. As a company that values human empowerment and as we think about what it means to “create renewable human energy (– Kathleen Hogan)”, the youth population is a crucial investment opportunity for the future. 


==> sections/old_section/03_youthwelltech_old.tex <==
\section{Youth WellTech} % method

\subsubsection{What is Youth WellTech}

Youth WellTech Collective is an advisory board consisting of youth participants distributed globally that provides expertise and guidance for technology design for the well-being of the youth population. The members of the collective are empowered with human-centered design practices and research mentors to investigate youth well-being challenges and to co-design future technology solutions to address them.

The program objectives are:
\begin{itemize}
    \item Co-design for youth with youth. Success means that the cohort generates an artifact aimed at improving the mental health and well-being of the youth population.
    \item Empower youth with human-centered design (HCD) skills. Success means that the cohort reports that they have gained knowledge and self-confidence in applying HCD skills to real-world problems.
    \item Empower youth to contribute to academic research or public discourse. Success means that the cohort can publish research insights and disseminate their findings in an academic venue, blog posts, articles or any medium of their choice.
    \item Develop a pipeline and process for ongoing partnership with youth to address youth mental health and well-being through technology. Success means that we have identified what works and does not work in the pilot phase and that we can pitch for renewed/refined program with funding and resources.
\end{itemize}

\subsubsection{Co-design sprint}
The program structure is largely inspired by human-centered design process, specifically the design sprint -- a design process that was created by Google Ventures and has since been adopted by many organizations and design teams. 
A design sprint is a structured, time-boxed process for solving complex problems and developing new ideas in a fast and collaborative manner. It typically lasts five days and involves a small, cross-functional team of designers, developers, product managers, and other stakeholders. in order to come up with a testable prototype that addresses a specific problem or challenge. In this study, the design sprint process involves the following steps:

\begin{itemize}
    \item Understand: The team spends the first day of the sprint understanding the problem or challenge and gathering insights through research and interviews.
    \item Define: The team identifies the most important challenge or opportunity and creates a clear goal for the sprint.
    \item Ideate: The team generates a wide range of ideas and potential solutions to the challenge.
    \item Prototype: The team creates a realistic and testable prototype of the best idea or solution.
    \item Test: The team tests the prototype with users to get feedback and validate assumptions.
\end{itemize}

Our session schedule closely follows the design sprint process across eight two-hour sessions. However, there are two main differences. (1) We adapt the design sprint process for co-design, where the design process is a shared process where end-users or stakeholders are active participants in the design process to create a shared understanding of the problem, identify potential solutions, and develop and test prototypes. (2) We elevate the role of the end-users or stakeholders as co-researchers to democratize knowledge production~\cite{}, recognize their expertise and agency in the research and design process, and provide ownership over the research outcomes.

% Aims of Co-research:

% Democratize Knowledge Production:

% Cornwall, A., & Jewkes, R. (1995). What is participatory research?. Social science & medicine, 41(12), 1667-1676.
% Contextual Understanding:

% Green, L. W., & Mercer, S. L. (2001). Can public health researchers and agencies reconcile the push from funding bodies and the pull from communities?. American Journal of Public Health, 91(12), 1926-1929.
% Empowerment:

% Israel, B. A., Schulz, A. J., Parker, E. A., & Becker, A. B. (1998). Review of community-based research: assessing partnership approaches to improve public health. Annual review of public health, 19(1), 173-202.
% Inclusivity:

% Minkler, M. (2004). Ethical challenges for the “outside” researcher in community-based participatory research. Health education & behavior, 31(6), 684-697.
% Enhancing Relevance:

% Wallerstein, N., & Duran, B. (2006). Using community-based participatory research to address health disparities. Health promotion practice, 7(3), 312-323.
% Benefits of Co-research:

% Richer Data:

% Jagosh, J., Macaulay, A. C., Pluye, P., Salsberg, J., Bush, P. L., Henderson, J., ... & Greenhalgh, T. (2012). Uncovering the benefits of participatory research: implications of a realist review for health research and practice. Milbank Quarterly, 90(2), 311-346.
% Increased Trust:

% Horowitz, C. R., Robinson, M., & Seifer, S. (2009). Community-based participatory research from the margin to the mainstream: are researchers prepared?. Circulation, 119(19), 2633-2642.
% Enhanced Validity:

% Cargo, M., & Mercer, S. L. (2008). The value and challenges of participatory research: strengthening its practice. Annual review of public health, 29, 325-350.
% Capacity Building:

% Israel, B. A., Eng, E., Schulz, A. J., & Parker, E. A. (Eds.). (2012). Methods for community-based participatory research for health. John Wiley & Sons.
% Ethical Research:

% Flicker, S., & Nixon, S. A. (2015). The DE-PHA-stated—a definition, a reflection, and a table. In Participatory qualitative research methodologies in health (pp. 1-17). Sage Publications Ltd.
% Community Ownership:

% Israel, B. A., Checkoway, B., Schulz, A., & Zimmerman, M. (1994). Health education and community empowerment: conceptualizing and measuring perceptions of individual, organizational, and community control. Health education & behavior, 21(2), 149-170.
% Innovation:

% Viswanathan, M., Ammerman, A., Eng, E., Garlehner, G., Lohr, K. N., Griffith, D., ... & Whitener, L. (2004). Community‐based participatory research: assessing the evidence. Evidence report/technology assessment (Summary), (99), 1.




% Challenges of co-research

\subsubsection{Program overview} % Kenji
%Summary of how youth welltech sessions were conducted

% \iffalse
% Week 1

% - Introduction and program overview, everyone introduced themselves, we learned about the codesign workflow, Human centered design, design sprints, how to use figJam etc
% - An activity to envision technology utopia and dystopia for mental health and wellbeing by putting down their thoughts in note cards on a figJam whiteboard
% - An activity to discuss the mental health and wellbeing challenges, plotted affinity diagrams from students thoughts
% - Draft the problem statement for mental health and wellbeing issues in youths
% - Students homework: background research on a self selected topic within the mental health and wellbeing space for youths

% Week 2
% - Reflection on individuals and shared goals, we wanted to identify what we want to achieve by the end of the project
% - Went through background research homework on week 1 and discussed
% - Refine problem statement
% - Learned about HMW (How might we) technique and used them to brainstorm about how might we solve the mental health and wellbeing issues amongst youths
% - Built upon the "how might we"s with the Golden Circle technique by Simon Sinek - Whys (why does this problem matter, why are we solving it), Hows (what's our approach, how to scope it and constraints) and What (what is our success criteria, what are our stated ambitions/intentions)
% - Had an activity about our inspirations, students and researchers shared content that inspired them
% - Had another homework for background research on how we might be able to solve this problem

% Week 3
% - Discussed background research from week 2
% - Learned about technique and flow of how to break down a problem and how to solve it
% - Had some fun with Skribble.io
% - Learned about 4 step sketching
%   - Gather key info
%   - Doodle rough solutions
%   - Try rapid variations
%   - Figure out the details
% - Homework: Students had homework to sketch a solution, produce a comic like user story on the problem and a solution

% Week 4
% - Went through students homework, their sketches
% - Learned about prototyping and scoping
%   - Paper prototypes
%   - Wireframes
%   - UI mockups
%   - Figma
% - Students were split into 3 teams based on the most voted on solutions to explore which were 
%   - 1. Setting guardrails by filtering and restricting unhealthy social media content
%   - 2. Gamification on coping with social media addiction
%   - 3. Helping people do simple and important activities to keep them busy and productive
% - Learned about scoping and planning
% - Homework: Students in their teams had to build upon their sketches into prototypes, everyone agreed to use Figma

% Week 5
% - Ask me anything session with the researchers and students
% - Prototype showcase for each teams, others can note down their thoughts and questions while teams were presenting
% - Went through the thoughts and questions together
% - Learned about test planning as we needed a way to test if our prototypes' effectiveness
%   - think aloud approach
%   - user usage assessment test, test if flow is intuitive
% - Homework: teams were given a document template on how to come up with a test plan and had to finalize a test plan for the prototype

% Week 6
% - Members from each team would be paired with another member from another team and a user test session will be run between them on their respective prototypes

% Week 7
% - Researchers and participants decided on how to come up with a output for the design 
% - Participants choosed between making a blog / video or article, decided on making a video to showcase work
% - Learned about key techniques of making a good video pitch
% - Homework: Teams had to make a video of their output, video was set to be 10 minutes long, presented to the stakeholders of the student program with 5 minutes questions for each team

% Week 8
% - Teams presented their videos to key stakeholders of the program and got asked questions, researchers from the same research group as the organizers and project managers of the student program were among the attendees
% - Key stakeholders were satisfied with each of the projects presented
% \fi

% Turn these subsubsections into paragraphs - {new ones to be put here}
In the inaugural week of our 8-week co-design initiative, we initiated our expedition into the realm of co-design by acquainting ourselves with essential elements. Participants embarked on a voyage of exploration, which encompassed the exchange of introductions and an in-depth overview of the program's objectives. This phase was instrumental in establishing a comprehensive framework, underpinned by design principles such as Human-Centered Design (HCD) and the practical utilization of tools like FigJam.
 The journey in the first week not only set the stage for what lay ahead but also engaged us in discussions concerning the intersection of technology and mental health. Participants engaged in a thought-provoking activity that prompted them to envision both utopian and dystopian scenarios in the context of technology's impact on mental health and wellbeing. These insights, transcribed onto note cards on a FigJam whiteboard, played a pivotal role in framing and refining the problem statements we aimed to address.


In the second week, our focus shifted to a more structured understanding of collective goals and the problems we intended to address. We reflected on individual and shared objectives, laying the foundation for a comprehensive problem statement. Additionally, the group reviewed the background research conducted during the previous week. We introduced the "How Might We" (HMW) technique, a cornerstone of design thinking, to catalyze ideation. Participants utilized HMW questions to brainstorm potential solutions to the challenges related to youth mental health and wellbeing. Building upon these ideations, we incorporated Simon Sinek's Golden Circle framework, which enabled us to delve into the 'Whys' (the significance of the problem), 'Hows' (approach and constraints), and 'What' (success criteria and intentions) of our proposed solutions.The week also featured an activity where participants shared content that had inspired them, fostering a creative and collaborative atmosphere. Homework assignments were assigned, with participants tasked with conducting background research related to the potential solutions they had brainstormed.

In the third week, our discussions revolved around the synthesis of background research conducted during the previous week. We embraced techniques for breaking down complex problems into manageable components and devising solutions.A creative interlude featured a session of Skribble.io, encouraging participants to unwind while nurturing camaraderie. Subsequently, we dived into the '4 Step Sketching' technique, a storytelling approach that enabled the visualization of problem scenarios and potential solutions.Homework for this week required participants to sketch a solution, craft a comic-like user story depicting the problem and its resolution, and further explore their understanding of the problem space.


Week four marked a significant phase in our journey as we transitioned into the realm of prototyping and solution scoping. We reviewed and discussed the sketches submitted by participants during the previous week.Our exploration of prototyping encompassed various stages, including paper prototypes, wireframes, and UI mockups, with an emphasis on leveraging the Figma tool for digital prototyping. To further refine our focus, participants were divided into three teams based on the most favored solutions:

Setting guardrails through the filtration of unhealthy social media content.Implementing gamification to address social media addiction.Facilitating engagement in simple and meaningful activities to enhance productivity.With an understanding of our chosen directions, we proceeded to explore the intricacies of solution scoping and planning.

Homework assignments were distributed, tasking participants with elevating their initial sketches into detailed prototypes, utilizing the Figma platform for collaborative design

During the fifth week, we introduced testing methodologies to evaluate the effectiveness of our prototypes. Participants were acquainted with techniques such as the 'Think Aloud' approach, which emphasizes user engagement and feedback collection. This iterative process led to valuable refinements in our designs.Furthermore, we engaged in intra-group testing sessions where participants scrutinized and provided constructive feedback on other teams' prototypes. These sessions facilitated cross-pollination of ideas and fostered a spirit of collaboration.Homework for this week involved the development of comprehensive test plans for evaluating the prototype solutions.

The penultimate week witnessed the collective decision to transform our conceptualized solutions into tangible outputs. Participants opted for video presentations as the preferred format, a decision informed by the desire to enhance video pitch creation and communication skills. This choice was motivated by the objective of creating impactful, accessible, and engaging content.In addition to output selection, we delved into the essential techniques of crafting effective video pitches.

The culmination of our journey occurred in the eighth week when teams presented their meticulously produced videos to key program stakeholders. These stakeholders included research leaders, organizers, and project managers, ensuring a comprehensive review of our work. Each presentation provided an overview of our design journey and showcased the solutions we had diligently developed.The satisfaction expressed by key stakeholders underscored the success of our co-design approach and the impactful outcomes achieved throughout our 8-week endeavor.

\subsubsection{Participants}

\subsubsection{Method / study protocol} \jina{I can take a stab}

\todo{recruitment}
- Sent out a call for participation to Microsoft Learn Student Ambassador Gold member email list.
- The application asked to provide a brief statement on an area of youth mental health that they would like to explore and why, their time availability, basic demographics (age, gender, education), and whether they have prior experience in human-centered design or mental health related course or research work.
- Received 48 applications.
- Three organizers iteratively scored the applications on 3 dimensions: (1) how well they expressed their passion for MH in their statement, (2) the feasibility of the proposed approach in their statement, and (3) general time availability for sessions. 
- Taking from the ranked list based on scores, we maximized the diversity on gender identity and country of origin.
- Invited 15 applicants and 12 consented to participate.

\todo{facilitation/communication, including Teams communication}

\todo{tools we used, Figjam/powerpoint/Teams and etc.}

\todo{measurement instruments, weekly and study-wide reflections}







\subsection{Summary of the outputs}

%Yousra/Chino: SMT
\subsubsection{Social Media Tracker}

%SMT idea and need
As young individuals, especially students, are continually exposed to an abundance of streamed content through various social networks on a daily basis, it becomes imperative to address the potential negative consequences of excessive social media use. To tackle this issue, we introduce the Social Media Tracker (SMT) – a mobile application designed to mitigate the time spent on social media platforms. SMT provides users with the tools to monitor and regulate their social media activity through the incorporation of built-in time and content filters. Furthermore, the system incentivizes users through rewards based on their achievements in time-limited challenges.

Our hypothesis posits that such a strategic intervention can be instrumental in fostering healthier social media usage patterns among youth. By limiting digital dependency and promoting responsible usage, we aim to contribute positively to their mental well-being. SMT empowers young individuals to track their daily social media consumption, utilizing time filters to curtail excess usage and providing notifications if necessary. Additionally, users can personalize their visible social media content with the aid of mental health tips integrated into the app.

%SMT features
% Make this into a paragraph

%Kenji: 
\subsubsection{LifeQuest}
LifeQuest represents a gamified productivity application developed to address the escalating issue of excessive consumption of detrimental social media content, with a specific focus on YouTube.The core concept of the app revolves around "quests," which draws inspiration from traditional gaming while mirroring the real-life objectives and activities of the user. When a user selects a task from their to-do list, LifeQuest diligently monitors their YouTube usage, employing AI to analyze video metadata. As users remain aligned with their chosen objectives, they are rewarded with points as positive reinforcement.However, if the content deviates from the selected task, users lose lives, akin to the mechanics found in classic video games. When all lives are depleted, a custom-tailored motivational message is displayed, serving as a reminder of the user's original purpose for using the app.LifeQuest empowers young individuals to cultivate mindful content consumption, ensuring that their goals remain at the forefront while fostering resistance to the temptation of consuming unhealthy videos. It transforms the process into a game-like experience, encouraging users to approach their digital consumption with purpose and intention.

%\begin{itemize}
%\item : Promotes users to engage with useful and goal-aligned content on YouTube.
 %   \item Strengthen Resistance to Unhealthy Content Temptations: Builds resilience and self-control, reducing the 
  %  \item Save Time for Increased Productivity: Enables users to redirect saved time towards more meaningful tasks.
   % \item Attain Personalized Motivation and Feedback for continuous improvement
   % \item Enjoy the process: Treat the process like a game
%\end{itemize}

\subsubsection{ImpAct}
ImpAct is a mobile application designed to propose a digital way of prioritizing mental wellness. The primary objective of ImpAct is to encourage individuals to proactively invest in their mental health by breaking away from their routine and exploring new activities and experiences. By doing so, the application aims to promote a balanced approach to mental wellness, a facet of health that is often neglected.
The app displays a list of activities can range from novel experiences to activities that users may have never attempted before. To ensure sustained engagement and interest in these tasks, the application leverages Generative AI technologyGenerative AI comes into the picture, providing users with detailed and visual guidance on how to successfully complete the tasks especially when its being done for the first time.











==> sections/old_section/04_findings_notes.tex <==

\section {Challenges covered - Unofficial, its just notes}
Tokenism
Earlier Mention: The issue of equal participation in co-design, where some participants might feel they are contributing just for the sake of it without their inputs being genuinely considered, connects with the concept of tokenism.
Power Dynamics
Earlier Mention: When discussing the challenges of certain participants dominating the discourse, this can be seen as a manifestation of power dynamics, where certain voices overshadow others.
Insufficient Training
Earlier Mention: The aspect where participants were unfamiliar with concepts like co-design, HCI, or human-centered design and hence might not be able to contribute effectively.
Ethical Concerns
Earlier Mention: The potential for participants to drop out or be replaced might touch upon ethical concerns, especially if the reasons for their discontinuation aren't addressed appropriately.
Time and Resources
Earlier Mention: The challenge of participants being busy with their personal commitments and the necessity for them to prioritize the co-design program.
Unresolved Conflicts
Earlier Mention: The potential for disagreements when certain participants dominate or when there's a misalignment of goals.
Cultural Insensitivity
Earlier Mention: The emphasis on inclusivity and understanding diverse perspectives can be related to the challenge of cultural insensitivity.
Overburdening Participants
Earlier Mention: Some participants felt the workload was more intensive than anticipated, suggesting that they might have felt overburdened.
Inadequate Recognition
Earlier Mention: While not directly mentioned, ensuring participants felt valued and recognized for their unique contributions was a recurring theme.

\section {quotes that can easily be used - Unofficial, its just notes}
Misalignment & Unfamiliarity with Design and Research
"...a little concern about fitting in since design isn't really my expertise. I prefer coding."
"...I sometimes feel that we still need some time to discuss the ideas we had but we directly start brainstorming on the next step without having a real discussion."
"...it would be interesting to identify the relationships between the different problems, finding a root cause and a pain point."
"Unresponsive teammates"
Positive Experiences
"Discussion and engagement activities were amazing I even didn't realise 2 hours pass."
"It was great Introductory session. I have been getting answers to my questions with clear objectivity."
"It's a human nature we invest those things which benefit us so before every activity if we get to know how it will benefit us."
"So far, so good. I am learning about things related to UX and mental health, including approaches to enhance my career towards research."
Time Constraints and Pacing
"According to my view time slot given for activities were less but although it was great."
"We can increase the session duration. Like, In the previous session, we had to wrap up real quick when things just started to get interesting."
"Timing, we went over the time on some sections, too little time for some thinking exercises."
"Maybe more time? or less activities with more focus on them."
Engagement & Interactivity
"It's eye opening, encouraging and insightful to know that people are concerned about the impact of technology to our mental health."
"The role of moderators in incentivizing participation. Being clear with what is expected from us in every task of the day."
"So far, so good. Personally, I've wanted to dedicate more time to the program outside the sessions to learn more about the topics we're working on and be able to provide more relevant knowledge to the program."
The teamwork and work organization. I also like the idea when we synthesized each brainstorming step and interpreted the ideas we collected as clusters.


\subsection{Participants enjoyed the program}
The program received enthusiastic feedback regarding its engaging nature. Participants expressed sentiments such as, "Discussion and engagement activities were amazing. I didn't even realize 2 hours passed. So much enthusiasm was there," and, "For start everything is good :D." Moreover, the interactive nature of the sessions was praised: "The teamwork, the brainstorming process, and using Figma to collaborate with my teammates" and "The challenges organized by the organizer were amazing."
\subsection{Participants learned something new}
The program served as a valuable learning experience. Participants gained knowledge in diverse areas, from technical tools like Figma to broader design processes. Comments included, "Learnt a lot of new things like FigJam is really nice to use" and "So far, so good. I am learning about things related to UX and mental health, including approaches to enhance my career towards research." The program was also highlighted as instrumental in refining ideas and enhancing thought processes.
\subsection{Participants got to discuss and exchange perspectives with others}
The platform facilitated in-depth discussions around youth mental health. One participant noted the importance of diverse representation: "I like that we were given an opportunity to voice our ideas but I am not confident that our solutions would cater to everyone." Another emphasized, "The voice of the youths were definitely heard. A lot of youth out there are looking for ways to deal with mental health and the solutions will be of great help to them."
\subsection{Participants felt supported throughout the program}
The support provided by the facilitators was a recurring theme in the feedback. A participant expressed, "It is very easy to reach out to anybody from the team of facilitators. I had a Q\&A with Ebele Okoli who provided great insights and resources."
\subsection{Participants felt empowered}
The program instilled a sense of empowerment among participants. When being asked about what went well with thr program, a feedback emphasized, "How you [the facilitator] are considering the voice of every individual." Moreover, the program's impact extended beyond the sessions, influencing participants' overall approach: "The program's emphasis on engagement and commitment has been particularly beneficial to me." And also spawned an unexpected blogpost series from one of the participants which was really unexpected.

==> sections/old_section/04_findingsold.tex <==
\section{Findings} % need better title / results

%% mauybe that we write one to one mapping for findings and guidelines in one section where we talk about one finding and one lesson learnt, and separate parts for each, or we do all findings and then 3 lessons learnt in the guidelines, depends, we don't know yet until the person writing this section decides.

\todo{Look at our collective experiences critically What worked and what didn't work for our youth welltech program %Kenji/Yousra/Marko 
- quantitative and qualitative data - Personal stories or group discussions, e.g. multiple timezones didn't work for us, or we learned human centered design that might have worked or didn't work (challenges in planning, in Oraganizing Community-based events in partipatory action research paper)}

\subsection{Reflections}

%Analyzing weekly reflections
At the end of each session, participants were asked to fill a weekly reflection form to collect feedback about the program. As the latter was 8 weeks long, the following table \ref{tab:participantsperweek} presents the distribution of the number of participants per week:

\begin{table}[h!]
\caption{Number of participants per week}
\centering
    \begin{tabular}{|p{1cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|}
        \hline
          Week & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8\\
        \hline
          Number & 10 & 8 & 6 & 5 & 7 & 9 & 4 & 10\\
        \hline
    \end{tabular}
    \label{tab:participantsperweek}
\end{table}

% What activities people engaged in
\subsubsection{Activities}
The co-design approach requires engaging all parties in the design process to gather ideas and feedback from youth for investigating youth challenges and finding required solutions, the participants worked on a set of activities during each session as part of the co-design sprint.
According to the weekly reflections, here are most of the activities that youth were performing to reach the program objectifs:
\begin{itemize}
    \item Navigation on Figma: The main ideation tool used is a collaborative web application for interface design called Figma. The tool presented a set of services that helped establish a good communication between the participants from the ideation phase to prototyping.
    \item Mental health problems ideation: As part of the youth, participants collected the most common mental health problems that youth tries to overcome. The ideation process is a creative way to gather all possible ideas through individual and collectif brainstorming, that goes through three stages: problem ideas generation, selection and development of the top three encountered problems.
    \item Solution ideation: The same problem ideation process was used for solution ideation to find solutions for each identified problem. A How Might We (HMW) method was also used to capture opportunities and take insights of all possible solutions that could be implemented to solve youth mental health problems.
    \item Background research: Doing background research is an essential step to gather existing information about the current research field. Participants were invited to look for any information that could help in solving the identified problems as well as new approaches that could have been applied to improve the program.
    \item Storyboards creation: One of the most appreciated experiences that the participants included in the weekly reflection forms are making storyboards as it was, for most of them, their first time making one. Storyboards are usually used to map scripts and stories that can be implemented as use cases later when developing the solution.
    \item Solution prototyping: Once participants completed brainstorming their solutions that tackle youth mental health problems, they worked on prototyping them. It was as well a first experience for most of the program participants who worked on creating UX screens for each of the three solutions.
    \item User experience testing: As stated in the co-design sprint, solutions were tested on youth in order to collect feedback and improve the solutions continously. The testing phase demanded high understanding of the prototypes as well as large communities that could give different feedbacks from final users.
\end{itemize}

% What was appreciated by the participants
\subsubsection{Appreciation}
Many program attributes were explicitely appreciated by participants and reported as part of the things that went well during the program and led to its success. We believe that such strategies are the key to participants' continous involvement in the co-design process as they felt that their feedbacks were considered and new actions were conducted to improve the program in each session.
Here are some of the things that the participants found going well during the sessions:
\begin{itemize}
    \item Engagement and discussion: the co-design process we emplemented encourages countinous discussion between the team members in order to establish a good communication. The participants affirmed that, the discussions that were conducted during and after the sessions helped them understand their tasks and encouraged them engaging more as all their questions were answered by the program moderators and principal researchers. They also appreciated getting to meet different people from all over the world and sharing their inspiration about solving mental health problems and what solutions work best for them or for people they know.
    \item Using easy management and planning tools: many tools were used during the co-design process such as FigJam and timers. FigJam and Microsoft teams allowed participants brainstorm collectively and share their ideas more easily. However planning tools such as timers were as well appreciated as they helped schedule tasks and keep track of time during the sessions.
    \item The brainstorming process: The co-design process presented a set of brainstorming steps that helped guide the work. The latter process started by ideating about the commong mental health problems that youth encounter, then refined two problem statements and voted collectively on one. The next step was deciding core 'How Might We' solutions to tackle the problem including what approach to use and what success criteria to set.
    \item Program moderation: Many participants appreciated how the program was moderated and well managed by principal researchers and co-moderators as they had necessary guidance to help them succeed their tasks during the co-design process.
    \item Fun activities: As the participants didn't know each other at the beginning of the program, moderators planned a set of fun activities in order to reduce stress, help participants integate in the team more efficiently and establish a better teamwork.
    \item Opportunity of learning: It was a first experience for many participants to work on designing a solution, to work on storyboards or prepare a prototype for their solutions. They appreciated the facts that they had the opportunity and adequate resources to learn new skills and experience new challenges they never had before.
\end{itemize}

% What did or didn't work
\subsubsection{Challenges}
Even all of these appreciation inputs, participants had some challenges during the program and some of them were tackled from session to another. Some of the challenges were commmunicational due to the remote participation mode and some were technical because of the participants choices.
\begin{itemize}
    \item At first, the problem statement was too vague and needed narrowing. Most of the participants felt lost in the two first sessions as the problem statement wasn't defined yet.
    \item Some participants found difficulties in interacting during the sessions which created awkward situations for the other participants. (e.g., no camera)
    \item Most of the participants found that the time allocated to the sessions was not enough for the activities and tasks that they had to complete.
    \item Since participants were students, they couldn't allocate more time to complete their work outside of the sessions because of their busy schedules.
    \item Technical issues were also encountered during the sessions due to connection issues and slow loading tools especially in the prototype testing phase.
\end{itemize}

% What improvements can be made
\subsubsection{Improvements}
In order to improve the co-design process and overcome these challenges, we have also sought participants help and collected their ideas for better results. The improvement suggestions were:
\begin{itemize}
    \item Extending the session duration and give more time to brainstorming activities.
    \item Presenting the overall session agenda at the beginning so that the participants can understand their tasks and be aware of the time allocated for each one.
    \item Sharing more research papers as references to learn more about mental health and improve the participants knowledge in the field, as well as bringing psychology science to the scope.
    \item Another suggestion was about assigning tasks to individuals so that everyone works on a specific activity then present the findings and discuss it with the group.
    \item Finally, some participants suggested finding a way to reach larger audience to gather more feedback.
\end{itemize}


% 



\todo{- Building in public (linked in posts) Challenges 
- e.g. cohort not being faimilar with each other or not feeling comfortable to speak up at the beginning
- difficulty in internet, breaking up conneciton, etc. Before During - Participation After - Supporting beyond prototype - Supporting research}


\subsection{Jina's findings}
\begin{itemize}
    \item finding 1
\end{itemize}

\subsection{Salman's findings (videos 1-4)}
\begin{itemize}
    \item Student Ambassadors were less vocal at the beginning, no one turned on their cameras.
    \item Addressing the elephant in the room, maybe it may seem like we want everyone to seem professional but we do not, helped make students feel more comfortable.
    \item Turning on cameras makes it feel more like a group of people talking and co-designing, an aspect which may be missed virtually without this. \jina{This could be quantified. Who's speaking for how long? Percentage of people with cameras on per session.}
    \item Challenge of internet connectivity being flakey
    \item Introducing games or some way to break the ice can help unify the group
\end{itemize}

% discussion on findings


\subsection{Marko's findings (videos 5-8)}
\begin{itemize}
    \item Ask question and Scribbler game in the beginning of the sessions let participants to meet each other more and somehow feel more comfortable/connected.
    \item Most of the sessions run out of time in the end, especially for some brainstorming  activities or things that needed more time. \jina{this can be quantified}
    \item It was more understandable that the final solution will be findings and/or mock-up/prototype. -> it was more clear what the outcome of the sessions were
    
\end{itemize}

\subsection{Chino's findings}
\begin{itemize}
    \item By including motivations in the solution, 35\% of youth mental health problems can be effectively solved, according to the majority of participants. \jina{try to clarify and bring evidence to this point}
    \item Insufficient time was devoted to brainstorming additional solutions.
    \item We wish we had more time and opportunity to work more and improve the solutions we worked on.
    
\end{itemize}


